The Many Moods of Emotion

This paper presents a novel approach to the facial expression generation problem. Building upon the assumption of the psychological community that emotion is intrinsically continuous, we first design our own continuous emotion representation with a 3-dimensional latent space issued from a neural network trained on discrete emotion classification. The so-obtained representation can be used to annotate large in the wild datasets and later used to trained a Generative Adversarial Network. We first show that our model is able to map back to discrete emotion classes with a objectively and subjectively better quality of the images than usual discrete approaches. But also that we are able to pave the larger space of possible facial expressions, generating the many moods of emotion. Moreover, two axis in this space may be found to generate similar expression changes as in traditional continuous representations such as arousal-valence. Finally we show from visual interpretation, that the third remaining dimension is highly related to the well-known dominance dimension from psychology.

==> plan.tex <==
Intro:
- Motivation: to find a bridge between psychological interpretations and affective computing.

Performance is going higher and higher in affective computing, especially in discrete emotion recognition. 
Many applications
But perf saturating
Small corpus : using GAN to augment dataset.
But more data now.
GAN useful for visual analysis. 
Important to understand what we are manipulating
Important to build link between representations
Generation of fac expression 

Affective computing is a topic of broad interest, finding applications in many fields such as health-care, marketing or human-machine interfaces. 
Therefore, a great effort has been put in the recognition of emotion across different contents. Indeed, several works propose to analyze facial expressions from images~\cite{dhall_static_2011,goodfellow2014generative, ng_deep_2015,acharya_covariance_2018}, from multimodal videos~\cite{ringeval2017avec,vielzeuf2017temporal,knyazev2017convolutional, dhall2018emotiw} or from multi-view videos~\cite{valstar2017fera,batista2017aumpnet}. Other works focus more on text~\cite{cambria2016affective,poria2016fusing, rosenthal2017semeval} or audio~\cite{schuller2013interspeech, schuller2018interspeech,huang2018speech}, finally building a very large and complete set of emotion recognition methods. 
Nevertheless, some recent works~\cite{vielzeuf2018occam} underline that the performance may begin to saturate on the emotion recognition task, because of the nature of the used datasets and of the subjective representation of emotion.

Thus, understanding and manipulating the emotion representation is of tremendous interest to progress towards a more complete affective computing ability. 
For that, the very definition of the facial expression of the emotion has to be defined. The literature comes up with three main definitions. First, Ekman \textit{et al.}~\cite{ekman_constants_1971} proposes discrete emotions, identifying six universal classes of emotion (e.g. "Happy", "Sad" or "Angry"). Later, the arousal-valence system was built by Russell, placing emotions in a 2-d continuous space. Finally, the Facial Action Coding Systems allows to objectively represent facial expression with Action Units (e.g. "raised eyebrow") and thus may be used to infer the emotion.

As the face is one of the main ways of expressing emotion, a branch of the affective computing community proposes to focus on the generation of facial expression, thus aiming at both a better interpretation of the visual consequences of an emotion representation and a straight-forward way to simulate emotion.
To solve this generation task, the computer graphics community focus on the animation of the faces with model-based approaches~\cite{soladie2013invariant, weber2018unsupervised, kim2018deep}. More recently deep learning approaches and especially Generative Adversarial Networks~\cite{goodfellow2014generative,choi2017stargan,tulyakov2017mocogan, ding2017exprgan, qiao2018emotional} have been proposed, still borrowing ideas to the computer graphics community~\cite{song2017geometry,pumarola2018ganimation} but also aiming to learn these facial expressions from diverse datasets and representations. 
Nevertheless, these approaches often are trained on small corpus recorded in controlled conditions and annotated with discrete emotions~\cite{lyons1998japanese,lucey2010extended, zhao2011facial}, meaning that the space of possible generated expressions is limited.

\begin{figure}[hb]
    \centering
    \includegraphics[width=\linewidth]{figures/3moods.pdf}
    \caption{Illustration of our 3-d representation space of emotion. The upper left figure shows the three planes along the three dimensions. Each plane is colored with the associated discrete classes of emotions. The planes with the generated expressions are provided in the three other quarters, showing the many possible moods inside a single class. Note that expressions in these three planes are only a part of the possible samples generated by our model. Better viewed in color.}
    \label{fig:manymoods}
\end{figure}

Even if larger in the wild corpus using other emotion representations such as action units or arousal valence exist~\cite{li_reliable_2017,benitez-quiroz_emotionet:_2016,mollahosseini_affectnet:_2017}, they are only used by a few authors~\cite{pumarola2018ganimation}. Moreover, the annotation cost of such representation is really higher than for discrete emotion. 

Last but but not the least, the described approaches are often focusing on the quality of the generated faces. 
In this paper, we propose to add another concern, building a bridge between psychological interpretations of the emotion representation and what is visually observed. 
Our contribution is therefore to propose a 3-dimensional representation of emotion based on the latent space a of neural network. This model is trained on discrete emotion classification and thus required less annotation effort than for traditional continuous approaches. 
Using it to annotate a large in the wild corpus, we then learn a generative adversarial network on the so-obtained dataset. We show that not only the generation of faces is more robust than with other representations, but also that the third dimension is visually in line with the psychological definition of dominance, enabling easy interpretations of the observed improvements.






Human communication is based on language, but also heavily relies on the body expression and especially on the face. Therefore automating the facial expression recognition is of great interest and find many applications, from marketing to health-care. 

It is the reason why during the past years many improvements in performance have been done with the emergence of deep learning methods and larger datasets. Several works even highlight the fact that the accuracy on different benchmarks may be saturating. 
To continue to improve the quality of the representations learned by the neural networks, a common trend of research is to constrain the internal representation of the network\cite{otberdout2018deep,acharya_covariance_2018,cai2018island} in order to create some important characteristics for emotion representation, such as compactness of the different classes. 

Another promising path of research is the generation of facial expressions. This allows to first visually interpret the neural network outputs and thus, check intra-class consistency, identify datasets biases, and better understand difficult samples. It may also be of real interest for concrete applications, such as in post-traumatic therapy where giving the patient a more positive reflect of oneself is a milestone to reach.

But before generating a facial expression from an original image, the very definition of the facial expression of the emotion has to be defined. The literature comes up with three main definitions. First, Ekman \textit{et al.}~\cite{ekman_constants_1971} proposes discrete emotions, identifying six universal classes of emotion (e.g. "Happy", "Sad" or "Angry"). Later, the arousal-valence system was built by Russell, placing emotions in a 2-d continuous space. Finally, the Facial Action Coding Systems allows to objectively represent facial expression with Action Units (e.g. "raised eyebrow") and thus may be used to infer the emotion.

\begin{figure}[hb]
    \centering
    \includegraphics[width=\linewidth]{figures/3moods.pdf}
    \caption{Illustration of our 3-d representation space of emotion. The upper left figure shows the three planes along the three dimensions. Each plane is colored with the associated discrete classes of emotions. The planes with the generated expressions are provided in the three other quarters, showing the many possible moods inside a single class. Note that expressions in these three planes are only a part of the possible samples generated by our model. Better viewed in color.}
    \label{fig:manymoods}
\end{figure}
Associated with these representations, diverse datasets may be found. Large datasets for discrete emotion are relatively numerous, as the annotation process is easier. JAFFE~\cite{lyons1998japanese} and Extended Cohn-Kanade~\cite{lucey2010extended} gathers respectively 213 and 1917 faces recorded in controlled conditions while  SFEW~\cite{dhall_static_2011}, Oulu-Casia~\cite{zhao2011facial}, FER2013~\cite{}, RAF~ and AffectNet respectively gathers 700, 1440, 32000, 20000 and 480000 faces recorded in uncontrolled conditions. For static images, the only large dataset manually annotated in arousal valence is AffectNet~\cite{mollahosseini_affectnet:_2017}. Finally, action units are available on several datasets, such as Extended Cohn-Kanade and Emotionet (around one million samples, but semi-supervised annotation).

To concretely modify the expression of a given face, the computer graphics community proposes very efficient approaches based on face modeling. Indeed, Soladié~\textit{et al.}~\cite{soladie2013invariant} uses a 4-d emotion representation space to animate face and Active-Appearance Models features. Later, Weber \textit{et al.}~\cite{weber2018unsupervised} proposes an unsupervised person-specific model, enabling to easily adapt the manifold to the targeted subject. Other more general works in animations enable to generate face animation from another example, as done by Kim \textit{et al.}~\cite{kim2018deep}.

But to really allow a person-independent framework, many other recent approaches focus on Generative Adversarial Networks~\cite{goodfellow2014generative}. Thus, Choi \textit{et. al}~\cite{choi2017stargan} propose a multi-domain approach, learning both facial attribute transfer and facial expression generation, while Quia \textit{et al.}~\cite{qiao2018emotional} use facial landmarks to improve the smoothness of a changing emotion. 
Another approach~\cite{song2017geometry} is using fiducial points to geometrically control the face animation while Tulyakov \textit{et al.}~\cite{tulyakov2017mocogan} is learning to directly generate sequences of images, based on a "content and motion" approach.

The aforementioned approaches are performed in controlled conditions and therefore are applied on small datasets. Moreover, the used emotion representation is mostly discrete, defined by basic emotions. When it is not the case, approaches are often model-based and thus difficult to generalize on other subjects.
Therefore, these methods limitations raised several questions. Should not we be able to cope with faces recorded in the wild when generating emotion ? But then how to handle the intrinsic continuous nature of emotion ? Finally, in such a case, how to interpret the representation manifold used to generate the continuous emotion ?

In this paper, we propose a 3-dimensional representation of emotion based on the hidden representation of neural network trained on discrete emotion classification and thus requiring less annotation effort than for traditional continuous approaches. Using it to annotate a large in the wild corpus, we then learn a GAN on the so-obtained dataset. We show that not only the generation of faces is more robust than with other representations, but also that the third dimension is visually in line with the psychological definition of dominance, enabling easy interpretations of the observed improvements.

